MSF-Model: Queuing-Based Analysis and Prediction of Metastable Failures in Replicated Storage Systems

Metastable failure is a recent abstraction of a pattern of failures that occurs frequently in real-world distributed storage systems. In this paper, we propose a formal analysis and modeling of metastable failures in replicated storage systems. We focus on a foundational problem in distributed systems -- the problem of consensus -- to have an impact on a large class of systems. Our main contribution is the development of a queuing-based analytical model, MSF-Model, that can be used to characterize and predict metastable failures. MSF-Model integrates novel modeling concepts that allow modeling metastable failures which was interactable to model prior to our work. We also perform real experiments to reproduce and validate our model. Our real experiments show that MSF-Model predicts metastable failures with high accuracy by comparing the real experiment with the predictions from the queuing-based model.

==> content/prediction.tex <==
\section{Prediction}

\tania{I am concerned about including this section in the paper. It would be cool to use prediction to enhance the QT approach, but this section actually replaces the whole algorithm presented in Section 4 for determining a MT failure. A reviewer would argue why all the QT, MC etc hassle if an LSTM can predict the metastable failure model}

\tania{It would be make more sense to include this into a "mitigation" approach}

Mitigating metastable failures involves predicting these failures before the system becomes overloaded with retry requests. By predicting a metastable failure, we can adapt the system's algorithmic policies or auto-scale the system to handle higher loads. In this section, we build on the lessons we learned from reproducing and modeling metastable failures and present a machine learning-based approach that predicts these failures using time-series prediction with Long Short-Term Memory (LSTM). %However, any state-of-the-art time-series prediction method can be implemented in this approach.

\subsection{Datasets}
\begin{table}[t]
    \caption{Overview of Datasets Parameters}
    \label{tab:datasets_parameters}
    \centering
    \begin{tabular}{lp{0.3\textwidth}}
        \hline
        \textbf{Category} & \textbf{Parameters} \\
        \hline
        Time Series & Time \\
        \hline
        Paxos Specific & Batch Size, Interval, Timeout, Latency, System Load, Goodput \\
        \hline
        Postgres Specific & Postgres Network, CPU, and Memory Usage \\
        \hline
        Node Specific & CPU Usage, Memory Usage, Network Usage, Disk Usage \\
        \hline
        JVM Specific & GC Usage, JVM Threads, JVM Blocked Threads, JVM Memory Usage \\
        \hline
    \end{tabular}
   
\end{table}

We utilized the prototype introduced in Section~\ref{sec:prototype} to generate multiple time-series datasets by including different types of features. These features were captured using the Prometheus monitoring system~\cite{bjorn2015prometheus}, a widely-used tool in industry settings. Each generated time-series dataset contains $55$ metrics categorized as shown in Table~\ref{tab:datasets_parameters}.
The prototype was used to replicate various metastable failures under different system configurations, resulting in distinct time-series datasets. These datasets, automatically generated using the Prometheus metric system, can be used for analyzing a wide-range of systems in the context of metastable failures.
 
Each dataset represents a time-series for an experiment following the ``Load Surge'' scenario, where the load increases for some time as triggering the event, and retry requests serve as a sustaining effect. Each data entry is labeled to indicate if a metastable failure will occur in the next $40$ seconds. The exact beginning time of a metastable failure can be calculated using the formalization introduced in~\cite{bronson2021metastable}.

\subsection{ML Model} 
\tania{How are the parameter values selected (window size, LSTM architecture)? We can add a line saying that we empirically found the best configuration...}
The machine learning (ML) model input is created by applying a sliding window of size $100$ to the time series data entries, where each window consists of a data matrix with dimensions $(100, 55)$, as each data entry includes $55$ features. The label for each window indicates whether a metastable failure will occur within the next $40$ seconds. The sliding window mechanism is a common technique in time-series prediction models~\cite{frank2001timeseries}.
%
Each input is then fed into an LSTM layer with a depth of $64$ for training. The output of the LSTM layer is subsequently passed to a Dense layer with a size of $8$ and a ReLU activation function to facilitate generalization. Finally, a sigmoid activation function predicts the probability of a metastable event occurring within the next $40$ seconds.

\tania{Why 40? It sounds very random. At least I would add plots for a range of horizon windows (10 sec, 20, 1 min, 2 min...)}
This ML model allows us to feed real-time data into the system in the form of sliding windows and make predictions for the next $40$ seconds. This can be utilized in the common monitoring systems in order to feed data in real-time into the trained ML model and use the prediction results to prevent a future metastable failure that might occur.   


\subsection{Evaluation}

Our proposed ML model was trained using the dataset generated from the scenario outlined in Section~\ref{sec:reproduction}. The dataset features request intervals and timeouts set at $300ms$ and $600ms$, respectively. The batch size was incrementally increased from $220 KB$ to a peak of $300 KB$. A metastable failure is triggered at time $10:13$. 
%
For training, all data points after time $09:33$ were labeled $1$ to signal an upcoming metastable failure within the ensuing $40$ seconds. Data points before this time were labeled as $0$.
%
The training involves $100$ epochs using the Adam optimization algorithm~\cite{kingma2014adam}, with mean squared error serving as the loss function.


\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/prediction.pdf}
	\caption{Prediction of occurring a metastable failure in the next $40$ seconds using LSTM model. }
	\label{fig:prediction}
\end{figure}

For testing, we used a separate dataset generated via the same prototype in a different experiment. In this dataset, the batch size was incrementally raised from $150 KB$, reaching a peak at $280 KB$, and then gradually decreased to a low of $25 KB$. All other configurations align with those of the training dataset.
%
Figure~\ref{fig:prediction} illustrates the ML model's predictions for this test set as related to the system load. In this prediction, data entries before time $13:44$ have a prediction label close to $0$, suggesting a low probability of a metastable failure occurring within the next $40$ seconds. Conversely, after this timestamp, the prediction label approaches $1$, indicating a high likelihood of a metastable failure occurring within the next $40$ seconds or that such a failure has already occurred.




